Accurate Sampling Timing Acquisition for Baseband OFDM Power-line Communication in Non-Gaussian Noise

In this paper, a novel technique is proposed to address the joint sampling timing acquisition for baseband and broadband power-line communication (BB-PLC) systems using Orthogonal-Frequency-Division-Multiplexing (OFDM), including the sampling phase offset (SPO) and the sampling clock offset (SCO). Under pairwise correlation and joint Gaussian assumption of received signals in frequency domain, an approximated form of the log-likelihood function is derived. Instead of a high complexity two-dimension grid-search on the likelihood function, a five-step method is employed for accurate estimations. Several variants are presented in the same framework with different complexities. Unlike conventional pilot-assisted schemes using the extra phase rotations within one OFDM block, the proposed technique turns to the phase rotations between adjacent OFDM blocks. Analytical expressions of the variances and biases are derived. Extensive simulation results indicate significant performance improvements over conventional schemes. Additionally, effects of several noise models including non-Gaussianity, cyclo-stationarity, and temporal correlation are analyzed and simulated. Robustness of the proposed technique against violation of the joint Gaussian assumption is also verified by simulations.

==> Biography.tex <==
%Chen Chen
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ChenChen_Bio}}]{Chen Chen}
received the B.S. degree in microelectronics from Fudan University, Shanghai, China, in 2010. He is currently working toward the M.S. degree in microelectronics at the State Key Laboratory of ASIC \& System, Fudan University, Shanghai, China. His research interests include advanced signal synchronization, cognitive radio, and MIMO techniques.   
\end{IEEEbiography}
%Yun Chen
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Yunchen_Bio}}]{Yun Chen}
(M'08) received the B.S. and M.S. degrees in microelectronics from UESTC, China, in 2001 and 2004, respectively, and the PhD. degree from Fudan University in 2007. Dr. Chen is currently a lecturer with the State Key Laboratory of ASIC \& System, Microelectronics Department, Fudan University, Shanghai, China. Her research interests include VLSI architectures and integrated circuit (IC) design for communications and digital signal processing systems. Resent years more than 30 Research papers are published in SCI journals or the International Conference. All these papers are about digital signal processing, digital TV, the FEC encoding and decoding. She serves as a member of the Technical Program Committee of the IEEE International Conference on ASIC in 2009 and reviewers of the IEEE the Trans on CAS-I, IEEE the Trans on VLSI, EUIP the signal processing, IET, etc.
\end{IEEEbiography}
%Na Ding
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{NaDing_Bio}}]{Na Ding}
received the B.S. degree in microelectronics from Fudan University, Shanghai, China, in 2011. She is currently working toward the M.S. degree in microelectronics at the State Key Laboratory of ASIC \& System, Fudan University, Shanghai, China. Her research interests include OFDM synchronization for advanced communication systems and algorithms in  optical fiber communication.
\end{IEEEbiography}
%Yizhi Wang
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Wyz_Bio}}]{Yizhi Wang}
received his B.S. in microelectronics from Fudan University in 2010. He is currently a Master candidate at Fudan University. His research interests include communications, signal processing and VLSI design.
\end{IEEEbiography}
%Jia-Chin Lin
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{JCL_Bio}}]{Jia-Chin Lin}
(S'95-M'98-SM'03) received a B.S. and a M.S. degree from the Department of Electronics Engineering at National Chiao Tung University (NCTU) in Taiwan in 1994 and 1995, respectively, and a Ph.D. degree from National Taiwan University (NTU) in Taiwan in 1998.

Jia-Chin Lin was in the obligatory military service from July 1998 to March 2000 and then joined the Microelectronics and Information Systems Research Center at NCTU as a Research Assistant Professor. In February 2001, he joined the Department of Electrical Engineering at National Chi Nan University (NCNU) in Taiwan as an Assistant Professor. In August 2004, he was promoted to serve as an Associate Professor. From July to August of 2004 and from August 2005 to July 2006, he held the visiting associate professorship in the Department of Electrical Engineering at Stanford University. In August 2006, he joined the faculty in the Department of Communication Engineering at National Central University (NCU) in Taiwan as an Associate Professor. In August 2008, he was promoted to serve as a Full Professor. In January 2011, he became a Distinguished Professor. Since August 2011, he has been serving as the Chairperson in the Department of Communication Engineering at NCU. His research interests include wireless transmission technologies, signal processing for communications and signal synchronization techniques.
\end{IEEEbiography}
%Xiaoyang Zeng
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Xiaoyangzeng_Bio}}]{Xiaoyang Zeng}
(M'05) received his PhD degree from Changchun Institute of Optics, Fine Mechanics and Physics, Chinese Academy of Sciences in 2001 and did his postdoctoral research at Fudan University during 2001-2003. He joined Fudan University as an associate professor in 2003, and became a full professor in 2007. His research interests include high-performance and energy-efficient SOC Integration, especially, VLSI designs for wireless communication ICs, information security ICs and mixed-signal ICs. He has published over 100 papers and applied for over 30 patents.
\end{IEEEbiography}
%Defeng (David) Huang
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{david_huang_Bio}}]{Defeng~(David)~Huang}
(M'01-S'02-M'05-SM'07) received the B. E. E. E. and M. E. E. E.
degree in electronic engineering from Tsinghua University,
Beijing, China, in 1996 and 1999, respectively, and the Ph.D.
degree in electrical and electronic engineering from the Hong Kong
University of Science and Technology (HKUST), Kowloon, Hong Kong,
in 2004.

Currently, he is a professor with the School of Electrical,
Electronic and Computer Engineering at the University of Western
Australia. Dr. Huang serves as an Editor for the IEEE
W\textsc{ireless} C\textsc{ommunications} L\textsc{etters}, he
also served as an Editor (2005-2011) for the IEEE
T\textsc{ransactions} \textsc{on} W\textsc{ireless}
C\textsc{ommunications}.
\end{IEEEbiography}

